A $\delta f$ PIC method with Forward-Backward Lagrangian reconstructions

In this work we describe a $\delta f$ particle simulation method where the bulk density is periodically remapped on a coarse spline grid using a Forward-Backward Lagrangian (FBL) approach. This method is designed to handle plasma regimes where the densities strongly deviate from their initial state and may evolve into general profiles. We describe the method in the case of an electrostatic particle-in-cell scheme and validate its qualitative properties using a classical two-stream instability subject to a uniform oscillating drive.

==> sources for arxiv R1/macros_fbl_df_pic.tex <==
% \usepackage[ansinew]{inputenc}
% \usepackage{amsmath,amssymb}
% \usepackage{amsthm}
% \usepackage{graphicx}
% \usepackage{bbm}
% \usepackage{bm}  % redefines \boldsymbol for better spacings, see http://tex.stackexchange.com/questions/3238/bm-package-versus-boldsymbol
% \usepackage{url}
% \usepackage{multirow}
% \usepackage{comment}
% \usepackage{tikz}
% %\usepackage{subcaption}

% \usepackage{framed}

% \usetikzlibrary{matrix}

% % \usepackage[right]{showlabels}
% %\usepackage{fancybox}
% \usepackage{algorithm}
% \usepackage{algorithmic}

\usepackage{booktabs}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

% \newcommand\blue[1]{{\color{blue} #1}}
% \newcommand\purple[1]{{\color{purple} #1}}



\def\loc{{\rm loc}}
\def\ext{{\rm ext}}
\def\ex{{\rm ex}}
\def\exa{{\rm ex}} % to remove it quickly if to needed
\def\bs{\boldsymbol}
\def\t{\tilde}
\def\wt{\widetilde}
\def\wh{\widehat}
\def\tbi{\t {\bs \imath}}
\def\ti{{\t \imath}}

\def\vp{{\varphi}}
\def\ve{{\varepsilon}}
\def\eps{{\epsilon}}

\def\Nppc{N_{\rm ppc}}

\def\bb{{\bs b}}
\def\bc{{\bs c}}
\def\bd{{\bs d}}
\def\be{{\bs e}}
\def\bi{{\bs i}}
\def\bj{{\bs j}}
\def\bm{{\bs m}}
\def\bn{{\bs n}}
\def\bq{{\bs q}}
\def\bu{{\bs u}}
\def\bv{{\bs v}}
\def\bw{{\bs w}}
\def\bx{{\bs x}}

\def\bA{{\bs A}}
\def\bB{{\bs B}}
\def\bC{{\bs C}}
\def\bD{{\bs D}}
\def\bE{{\bs E}}
\def\bF{{\bs F}}
\def\bH{{\bs H}}
\def\bJ{{\bs J}}
\def\bK{{\bs K}}
\def\bL{{\bs L}}
\def\bM{{\bs M}}
\def\bP{{\bs P}}
\def\bQ{{\bs Q}}
\def\bV{{\bs V}}
\def\bW{{\bs W}}
\def\bnabla{{\bs \nabla}}

\def\btau{{\bs \tau}}
\def\bvp{{\bs \varphi}}
\def\bpsi{{\bs \psi}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cI{\mathcal{I}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cJ{\mathcal{J}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cZ{\mathcal{Z}}

\def\bfx{{\bf x}}
\def\bfv{{\bf v}}
\def\bfz{{\bf z}}

\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfE{{\bf E}}
\def\bfJ{{\bf J}}
\def\bfM{{\bf M}}
\def\bfP{{\bf P}}
\def\bfF{{\bf F}}
\def\bfR{{\bf R}}
\def\bfX{{\bf X}}
\def\bfV{{\bf V}}
\def\bfW{{\bf W}}
\def\bfZ{{\bf Z}}

\def\bftA{\tilde {\bf A}}
\def\bftC{\tilde {\bf C}}
\def\bftM{\tilde {\bf M}}


% blackboard are sans-serif with \usepackage[bbgreekl]{mathbbol} of {upgreek}
\def\AA{\mathbb{A}}
\def\BB{\mathbb{B}}
\def\CC{\mathbb{C}}
\def\EE{\mathbb{E}}
\def\FF{\mathbb{F}}
\def\II{\mathbb{I}}
\def\JJ{\mathbb{J}}
\def\MM{\mathbb{M}}
\def\NN{\mathbb{N}}
\def\PP{\mathbb{P}}
\def\QQ{\mathbb{Q}}
\def\RR{\mathbb{R}}
\def\SS{\mathbb{S}}
\def\VV{\mathbb{V}}
\def\ZZ{\mathbb{Z}}

% bold blackboard fonts
% \mathbbm, \mathbbmss or \mathbbmtt with \usepackage{bbm}
\def\bAA{\mathbbm{A}}
\def\bCC{\mathbbm{C}}
\def\bNN{\mathbbm{N}}
\def\bRR{\mathbbm{R}}
\def\bZZ{\mathbbm{Z}}

\def\one{{\mathbbm{1}}}
\def\bfone{{\mathbf{1}}}
%\usepackage{relsize}
\usepackage{ esint }
\def\fintOm{{\fint_\Omega}}

\def\cNII{\cN^{\rm {II}}}
\def\cNI{\cN^{\rm {I}}}
\def\cRT{\mathcal{RT}}
\def\cBDM{\mathcal{BDM}}

\def\vol{{\rm vol}}
\def\face{{\rm face}}
\def\edge{{\rm edge}}
\def\vertex{{\rm vertex}}

\def\parts{{\rm parts}}
\def\pic{{\rm pic}}
\def\fbl{{\rm fbl}}
\def\ltp{{\rm ltp}}
\def\fsp{{\rm sp}}
\def\Ng{N_{\rm grid}}
\def\Nfbl{N_{\rm fbl}}
\def\Nproc{N_{\rm procs}}

\def\sfx{\mathsf{x}}
\def\sfv{\mathsf{v}}
\def\sfz{\mathsf{z}}
\def\sfA{\mathsf{A}}
\def\sfE{\mathsf{E}}
\def\sfM{\mathsf{M}}
\def\sfP{\mathsf{P}}
\def\sfT{\mathsf{T}}
\def\sfX{\mathsf{X}}
\def\sfV{\mathsf{V}}
\def\sfZ{\mathsf{Z}}


\def\Pe{{\sfP^{1}_{h,0}}}
\def\Pm{{\sfP^{0}_h}}

\def\Veh{V^\ve_h}
\def\tVeh{{\t V^\ve_h}}
\def\Vmh{V^\mu_h}
\def\tVmh{{\t V^{\mu}_h}}
\def\Vnuh{V^{\nu}_h}

\def\DG{{\rm DG}}
\def\pFE{{p_{\rm fe}}}
\def\pDG{{p_{\rm dg}}}

\def\intstepn{\int_{t^n}^{t^{n+1}}\mspace{-10mu}}
\def\rmd{\, {\rm d}} %for integrals
\def\Dt{{\Delta t}}
\def\Dx{{\Delta x}}
\def\Dy{{\Delta y}}
\def\Dv{{\Delta v}}
\def\dt{{\partial_{t}}}
\def\dx{{\partial_{x}}}
\def\dy{{\partial_{y}}}
\def\dv{{\partial_{v}}}
\def\dtt{{\partial^2_{t}}}

\def\df{{\delta f}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}


\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\bigabs}[1]{\big|#1\big|}
\providecommand{\Bigabs}[1]{\Big|#1\Big|}
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\bignorm}[1]{\big\|#1\big\|}
\providecommand{\Bignorm}[1]{\Big\|#1\Big\|}
\providecommand{\Norm}[1]{\left\lVert#1\right\rVert}

%\newcommand{\fracp}[2]{\frac{\partial #1}{\partial #2}}

\providecommand{\sprod}[2]{\langle#1,#2\rangle}
\providecommand{\Sprod}[2]{\left\langle#1,#2\right\rangle}

\providecommand{\average}[1]{\{\!\!\{#1\}\!\!\}}
\providecommand{\jump}[1]{[\![#1]\!]}

    % \usepackage{stmaryrd}
    %  \llbracket     1 \rrbracket       \quad
    %  \llparenthesis 2 \rrparenthesis   \quad
    %  \llceil        3 \rrceil          \quad
    %  \llfloor       4 \rrfloor         \quad


%\newcommand\purple[1]{{\color{purple} #1}}

\providecommand{\note}[1]{{\bf [note: #1]}}
\providecommand{\todo}[1]{{\bf To do}: {\em #1 }}

\def\blankfirst{\phantom{V^0} }
\def\blanksecond{\phantom{ \{ } } %\hspace*{-5pt}}


\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\gap}{gap}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\diag}{diag}

\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\rank}{rank}

\DeclareMathOperator{\tbcurlh}{\widetilde \bcurl_{\it h}}
\DeclareMathOperator{\tcurlh}{\widetilde \curl_{\it h}}
\DeclareMathOperator{\bcurlh}{\bcurl_{\it h}}
\DeclareMathOperator{\curlh}{\curl_{\it h}}
\DeclareMathOperator{\tcurlha}{\widetilde \curl_{\it h}^{\it a}}

\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\bcurl}{{\bf curl}}
%\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\bgrad}{{\bf grad}}

\DeclareMathOperator{\remap}{\mathsf{Remap}}
% \DeclareMathOperator{\deposit}{\mathsf{Deposit}}
% \DeclareMathOperator{\field}{\mathsf{Field}}
\DeclareMathOperator{\field}{\mathsf{E}}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{algo}[lemma]{Algorithm}
\newtheorem{problem}[lemma]{Problem}
%\newtheorem{todo}[lemma]{Todo}

% \newenvironment{proof}{\noindent{\it Proof. }}{\hfill\rule{2mm}{2mm}\vskip3mm
% \par}

\providecommand{\sprod}[2]{\langle#1,#2\rangle}



% \makeatletter
% \newcommand{\thickhline}{%
%     \noalign {\ifnum 0=`}\fi \hrule height 1pt
%     \futurelet \reserved@a \@xhline
% }
% \newcolumntype{"}{@{\hskip\tabcolsep\vrule width 1pt\hskip\tabcolsep}}
% \makeatother

